FinDVer: Explainable Claim Verification over Long and Hybrid-Content Financial Documents

We introduce FinDVer, a comprehensive benchmark specifically designed to evaluate the explainable claim verification capabilities of LLMs in the context of understanding and analyzing long, hybrid-content financial documents. FinDVer contains 2,400 expert-annotated examples, divided into three subsets: information extraction, numerical reasoning, and knowledge-intensive reasoning, each addressing common scenarios encountered in real-world financial contexts. We assess a broad spectrum of LLMs under long-context and RAG settings. Our results show that even the current best-performing system, GPT-4o, still lags behind human experts. We further provide in-depth analysis on long-context and RAG setting, Chain-of-Thought reasoning, and model reasoning errors, offering insights to drive future advancements. We believe that FinDVer can serve as a valuable benchmark for evaluating LLMs in claim verification over complex, expert-domain documents.

==> figures_tex/dataset_annotation_example.tex <==
\begin{figure}[!t]
    \centering
    \begin{tcolorbox}[colback=black!3!white, colframe=black!70!white, title=Example, fontupper=\footnotesize, fonttitle=\footnotesize]

\textbf{Claim:} 


\textbf{Supporting Paragraph Evidence Indices:} \newline [13, 14, 108, 110] \\

\textbf{Supporting Table Evidence Indices:} \newline [13, 14, 108, 110] \\

\textbf{Reasoning Process Explanation:} \\



\end{tcolorbox}
    \caption{\yilun{TODO} An example from the \mathset subset. We provide detailed annotation for the features of claim, supporting evidence, and reasoning-process explanation in a standardized step-by-step format.
    }
    \label{fig:solution_annotation}
\end{figure}
